Competing Bandits: The Perils of Exploration Under Competition

Most online platforms strive to learn from interactions with users, and many engage in exploration: making potentially suboptimal choices for the sake of acquiring new information. We study the interplay between exploration and competition: how such platforms balance the exploration for learning and the competition for users. Here users play three distinct roles: they are customers that generate revenue, they are sources of data for learning, and they are self-interested agents which choose among the competing platforms. We consider a stylized duopoly model in which two firms face the same multi-armed bandit problem. Users arrive one by one and choose between the two firms, so that each firm makes progress on its bandit problem only if it is chosen. Through a mix of theoretical results and numerical simulations, we study whether and to what extent competition incentivizes the adoption of better bandit algorithms, and whether it leads to welfare increases for users. We find that stark competition induces firms to commit to a "greedy" bandit algorithm that leads to low welfare. However, weakening competition by providing firms with some "free" users incentivizes better exploration strategies and increases welfare. We investigate two channels for weakening the competition: relaxing the rationality of users and giving one firm a first-mover advantage. Our findings are closely related to the "competition vs. innovation" relationship, and elucidate the first-mover advantage in the digital economy.

==> content/omitted_proofs.tex <==
\ascomment{This file is now obsolete!}

\subsection{Proof of Theorem~\ref{thm:HardMax-hardTies}}

\begin{proof}
The proof re-uses Lemmas~\ref{lm:DG-rew} and~\ref{lm:DG-sudden}, which do not rely on fair tie-breaking.

Because of the biased tie-breaking, for each global round $t$ we have:
\begin{align}\label{eq:thm:HardMax-biased-PMRtoPr}
\text{if $\PMR_1(t)\geq \PMR_2(t)$ then $\Pr[i_t=1]>\tfrac12$.}
\end{align}
Recall that $i_t$ is the principal chosen in global round $t$.

Let $m_0$ be the first step when \alg[2] deviates from \DynGreedy, or \DynGreedy deviates from \StaticGreedy, whichever comes sooner. \asedit{Then \alg[2], \DynGreedy and \StaticGreedy coincide on the first $m_0-1$ steps. Moreover, $m_0\leq n_0$ (since \DynGreedy deviates from \StaticGreedy at step $n_0$), so \alg[1] coincides with \DynGreedy on the first $m_0$ steps.

So, $\rew_1(n)=\rew_2(n)$ for each step $n<m_0$, because \alg[1] and \alg[2] coincide on the first $m_0-1$ steps. Moreover, if \alg[2] deviates from \DynGreedy at step $m_0$ then
    $\rew_1(m_0) > \rew_2(m_0)$
by Lemma~\ref{lm:DG-rew}; else, we trivially have
    $\rew_1(m_0) = \rew_2(m_0)$.} To summarize:
\begin{align}\label{eq:thm:HardMax-biased-rew}
    \rew_1(n)\geq\rew_2(n)\quad \text{for all steps $n\leq m_0$}.
\end{align}

We claim that $\Pr[i_t=1]>\tfrac12$ for all global rounds $t\leq m_0$. We prove this claim using induction on $t$. The base case $t=1$ holds by \eqref{eq:thm:HardMax-biased-PMRtoPr} and the fact that in step 1, \DynGreedy chooses the arm with the highest prior mean reward. For the induction step, we assume that $\Pr[i_t=1]>\tfrac12$ for all global rounds $t<t_0$, for some $t_0\leq  m_0$. It follows that distribution $\posteriorN{1}{t_0}$ stochastically dominates distribution $\posteriorN{2}{t_0}$.%
\footnote{For random variables $X,Y$ on \R, we say that $X$ \emph{stochastically dominates} $Y$ if $\Pr[X\geq x] \geq \Pr[Y\geq x]$ for any $x\in \R$.}
Observe that
\begin{align}\label{eq:thm:HardMax-biased-PMR-aux}
\PMR_1(t_0)
  = \Ex{n\sim \posteriorN{1}{t_0}} {\rew_1(n+1)}
  \geq \Ex{n\sim \posteriorN{2}{t_0}} {\rew_2(n+1)}
  = \PMR_2(t_0).
\end{align}
So the induction step follows by \eqref{eq:thm:HardMax-biased-PMRtoPr}. Claim proved.

Now let us focus on global round $m_0$, and denote $\mN_i = \posteriorN{i}{m_0}$.  By the above claim,
\begin{align}\label{eq:thm:HardMax-biased-mN}
\text{$\mN_1$ stochastically dominates $\mN_2$, and moreover
    $\mN_i(m_0-1)>\mN_i(m_0-1)$.}
\end{align}

By definition of $m_0$, either (i) \alg[2] deviates from \DynGreedy starting from local step $m_0$, which implies $\rew_1(m_0)> \rew_2(m_0)$ by Lemma~\ref{lm:DG-rew}, or (ii) \DynGreedy deviates from \StaticGreedy starting from local step $m_0$, which implies $\rew_1(m_0)>\rew_1(m_0-1)$ by Lemma~\ref{dgmono}. In both cases, using \eqref{eq:thm:HardMax-biased-rew} and \eqref{eq:thm:HardMax-biased-mN}, it follows that the inequality in \eqref{eq:thm:HardMax-biased-PMR-aux} is strict for $t_0=m_0$.

Therefore, agent $m_0$ chooses principal $1$, and by Lemma~\ref{lm:DG-sudden} so do all subsequent agents.
\end{proof}


\subsection{Proof of Theorem~\ref{thm:random-greedy}}
\begin{proof}
  Let $\rew'_1(n)$ denote the Bayesian-expected reward of the ``greedy
  choice'' after after $n-1$ steps of \alg[1]. Note that
  $\rew_1(\cdot)$ and $\rew'_1(\cdot)$ are non-decreasing: the former
  because \alg[1] is monotone and the latter because the ``greedy
  choice'' is only improved with an increasing set of
  observations. Therefore, the modified algorithm \alg[2] is monotone
  by \eqref{eq:random-BIR}.

  By definition of the ``greedy choice,'' $\rew_1(n)\leq \rew'_1(n)$
  for all steps $n$. Moreover, by Lemma~\ref{lm:DG-rew},
  \alg[1] has a strictly smaller $\rew(n_0)$ compared to \DynGreedy;
  so, $\rew_1(n_0)<\rew_2(n_0)$.

Let $\alg$ denote a copy of \alg[1] that is running ``inside" the modified algorithm \alg[2]. Let $m_2(t)$ be the number of global rounds before $t$ in which the agent chooses principal $2$ \emph{and} \alg is invoked; in other words, it is the number of agents seen by \alg before global round $t$. Let $\mM_{2,t}$ be the agents' posterior distribution for $m_2(t)$.

We claim that in each global round $t\geq n_0$, distribution $\mM_{2,t}$ stochastically dominates distribution $\posteriorN{1}{t}$, and $\PMR_1(t)<\PMR_2(t)$. We use induction on $t$. The base case $t=n_0$ holds because $\mM_{2,t} = \posteriorN{1}{t}$ (because the two algorithms coincide on the first $n_0-1$ steps), and $\PMR_1(n_0)<\PMR_2(n_0)$ is proved as in \eqref{eq:pf:thm:DG-dominance}, using the fact that $\rew_1(n_0)<\rew_2(n_0)$.

The induction step is proved as follows. The induction hypothesis for global round $t-1$ implies that agent $t-1$ is seen by \alg with probability $(1-\eps_0)(1-p)$, which is strictly larger than $\eps_0$, the probability with which this agent is seen by \alg[2]. Therefore, $\mM_{2,t}$ stochastically dominates $\posteriorN{1}{t}$.
\begin{align}
\PMR_1(t)
  &= \Ex{n\sim \posteriorN{1}{t}} {\rew_1(n+1)} \nonumber \\
  &\leq \Ex{m\sim \mM_{2,t}} {\rew_1(m+1)}
    \label{eq:pf:thm:random-greedy-1}\\
  &< \Ex{m\sim \mM_{2,t}} {(1-p)\cdot \rew_1(m+1) + p\cdot \rew'_1(m+1)}
    \label{eq:pf:thm:random-greedy-2} \\
  &= \PMR_2(t). \nonumber
\end{align}
Here inequality \eqref{eq:pf:thm:random-greedy-1} holds because $\rew_1(\cdot)$ is monotone and $\mM_{2,t}$ stochastically dominates $\posteriorN{1}{t}$, and inequality \eqref{eq:pf:thm:random-greedy-2} holds because $\rew_1(n_0)<\rew_2(n_0)$ and $\mM_{2,t}(n_0)>0$.%
\footnote{If $\rew_1(\cdot)$ is strictly increasing, then inequality \eqref{eq:pf:thm:random-greedy-1} is strict, too; this is because $\mM_{2,t}(t-1)>\posteriorN{1}{t}(t-1)$.  }
\end{proof}

\subsection{Proof of Theorem~\ref{thm:SoftMax-strong}}
\begin{proof}
  Let $\beta_1 = \min\{c_0'\delta_0, \beta_0/20\}$ with $\delta_0$
  defined in~\eqref{eq:SoftMax-smooth}.  Recall each agent chooses
  \alg[1] with probability at least $\respF(-1)= \eps_0$.  By
  condition \eqref{eq:so-mild} and \eqref{eq:SoftMax-assn-strong},
  there exists some sufficiently large $T_1$ such that for any
  $t\geq T_1$, $\BIR_1(\eps_0 T_1/2) \leq \beta_1/c_0'$ and
  $\BIR_2(t) > e^{-\eps_0 t/12}$. Moreover, for any $t\geq T_1$, we
  know $\E[n_1(t+1)] \geq \eps_0\,t $, and by the Chernoff Bounds
  (Theorem~\ref{thm:chernoff}), we have $n_1(t+1) \geq \eps_0 t/2$
  holds with probability at least $1 - q_1(t)$ with
  $q_1(t) = \exp(-\eps_0 t/12) < \BIR_2(t)$. It follows that for any $t\geq T_1$,
\begin{align*}
  \PMR_2(t) - \PMR_1(t) &= \Ex{m_1\sim \posteriorN{1}{t},\;m_2\sim \posteriorN{2}{t}}{\BIR_1(m_1+ 1) - \BIR_2(m_2+1)} \\
                        &\leq q_1(t)  + \Ex{m_1\sim \posteriorN{1}{t}}{\BIR_1(m_1+ 1)\mid m_1 \geq \eps_0 t/2 - 1 } - \BIR_2(t)\\
                        &\leq \BIR_1(\eps_0 T_1/2) \leq \beta_1/c_0'
\end{align*}
% where the second inequality follows from~\eqref{eq:random-assn}.
Since the response function $\respF$ is $c_0'$-Lipschitz in the
neighborhood of $[-\delta_0, \delta_0]$, each agent after round $T_1$
will choose \alg[1] with probability at least
\[
  p_t \geq \frac{1}{2} - c_0'\left(\PMR_2(t) - \PMR_1(t)\right) \geq
  \frac{1}{2} - \beta_1.
\]

Next, we will show that there exists a sufficiently large $T_2$ such
that for any $t\geq T_1 + T_2$, with high probability
$n_1(t) > \max\{n_0, (1 - \beta_0)n_2(t)\}$, where $n_0$ is defined
in~\eqref{eq:SoftMax-better}. %  Let us first lower bound the number of
% agents received by \alg[1] after some number of rounds $t = T_1 + T'$
% for any $T' \geq T_1$.
Fix any $t \geq T_1 + T_2$.
Since each agent chooses \alg[1] with probability at least
$1/2 - \beta_1$, by Chernoff Bounds (Theorem~\ref{thm:chernoff}) we
have with probability at least $1 - q_2(t)$ that the number of agents
that choose \alg[1] is at least $\beta_0(1/2 - \beta_1)t/5$, where the
function
$$
q_2(x) = \exp\left( \frac{-(1/2 - \beta_1)(1 - \beta_0/5)^2x}{3} \right).
$$
Note that the number of agents received by \alg[2] is at most
$T_1 + (1/2 + \beta_1)t + (1/2 - \beta_1)(1 - \beta_0/5)t$.

Then as long as
% $T_2 \geq \max\left\{\frac{3T_1}{(1 - \beta_0)}, 8 n_0\right\}$, we
% can guarantee that for any $t \geq T_1 + T_2$,
% $n_1(t) > n_2(t) (1 - \beta_0)$ and $n_1(t) > n_0$ with probability at
% least $1 - q_2(t)$.
$T_2 \geq \frac{5T_1}{\beta_0}$, we can guarantee that
$n_1(t) > n_2(t) (1 - \beta_0)$ and $n_1(t) > n_0$ with probability at
least $1 - q_2(t)$ for any $t \geq T_1 + T_2$.
% for any $t\geq T_1 + T_2$, as long as $T_2 \geq .$ Moreover, to
% guarantee that , we will just need $T_2 \geq$.  Finally, we will
% argue that in each round $t \geq T_1 + T_2$, we recover the
% guarantee in \eqref{eq:thm:SoftMax-strong}.
% % \[
% %   \Pr[i_t = 1] \geq \frac{1}{2} + \frac{c_0\alpha_0\BIR_2(t)}{4}.
% % \]
Note that the weak BIR-dominance condition
in~\eqref{eq:SoftMax-better} implies that for any $t\geq T_1 + T_2$
with probability at least $1 - q_2(t)$,
\[
  \BIR_1(n_1(t)) < (1- \alpha_0)\BIR_2(n_2(t)).
\]
It follows that for any $t\geq T_1 + T_2$,
\begin{align*}
  \PMR_1(t) - \PMR_2(t) &= \Ex{m_1\sim \posteriorN{1}{t},\;m_2\sim \posteriorN{2}{t}}{\BIR_2(m_2+ 1) - \BIR_1(m_1+1)} \\
                        &\geq (1 - q_2(t))\alpha_0 \BIR_2(t) - q_2(t)\\
                        &\geq \alpha_0 \BIR_2(t)/4
\end{align*}
where the last inequality holds as long as
$q_2(t) \leq \alpha_0\BIR_2(t)/4$, and is implied by the condition
in~\eqref{eq:SoftMax-assn-strong} as long as $T_2$ is sufficiently
large. Hence, by the definition of our \SoftMaxRandom response
function and assumption in~\eqref{eq:SoftMax-smooth}, we have
\[
  \Pr[i_t = 1] \geq \frac{1}{2} + \frac{c_0\alpha_0\BIR_2(t)}{4}. \qedhere
\]
\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:


==> itcs18paper/sec-intro.tex <==
Learning from interactions with users is ubiquitous in modern customer-facing systems, from product recommendations to web search to spam detection to content selection to fine-tuning the interface. Many systems purposefully implement \emph{exploration}: making potentially suboptimal choices for the sake of acquiring new information. Randomized controlled trials, a.k.a. A/B testing, are an industry standard, with a number of companies such as \emph{Optimizely} offering tools and platforms to facilitate them. Many companies use more sophisticated exploration methodologies based on \emph{multi-armed bandits}, a well-known theoretical framework for exploration and making decisions under uncertainty.

%~\cite{KohaviAB-2015,KohaviLSH09}

Systems that engage in exploration typically need to compete against one another; most importantly, they compete for users. This creates an interesting tension between \exploration and \competition. In a nutshell, while exploring may be essential for improving the service tomorrow, it may degrade quality and make users leave \emph{today}, in which case there will be no users to learn from! Thus, users play three distinct roles: they are customers that generate revenue, they generate data for the systems to learn from, and they are self-interested agents which choose among the competing systems.


We initiate a study of the interplay between \exploration and \competition. The main high-level question is: {\bf whether and to what extent competition incentivizes adoption of better exploration algorithms}. This translates into a number of more concrete questions. While it is commonly assumed that better learning technology always helps, is this so for our setting? In other words, would a better learning algorithm result in higher utility for a principal? Would it be used in an equilibrium of the ``competition game"? Also, does competition lead to better social welfare compared to a monopoly? We investigate these questions for several models, as we vary the capacity of users to make rational decisions (\rationality ) and the severity of competition between the learning systems (\competitiveness). The two are controlled by the same ``knob" in our models; \asedit{such coupling is not unusual in the literature, \eg see \citet{Gabaix-16}}.

\asedit{On a high level, our contributions can be framed in terms of the ``inverted-U relationship" between rationality/competitiveness and the quality of adopted algorithms (see \reffig{fig:inverted-U}).}

\OMIT{The relationship between the severity of competition among firms and the quality of technology adopted as a result of this competition is a familiar  theme in the economics literature, known as ``competition vs. innovation".%
\footnote{In this context, \innovation usually refers to adoption of a better technology as a substantial R\&D expense to a given firm. It is not as salient whether similar ideas and/or technologies already exist outside the firm. }
We frame our contributions in terms of the ``inverted-U relationship", a conventional wisdom regarding ``competition vs. innovation" (see \reffig{fig:inverted-U}).}

\begin{figure}
\begin{center}
\begin{tikzpicture}
      \draw[->] (-.5,0) -- (3,0) node[right] {Rationality/competitiveness};
      \draw[->] (0,-.5) -- (0,3) node[above] {Better algorithms};
      \draw[scale=0.6,domain=0.5:4.5,smooth,variable=\x,blue, line width=0.3mm] plot ({\x},{4.5 - (\x - 2.5)^2});
      % \draw[scale=0.5,domain=-3:3,smooth,variable=\y,red]  plot ({\y*\y},{\y});
 \end{tikzpicture}

\caption{Inverted-U relationship between rationality/competitiveness and algorithms.}
\label{fig:inverted-U}
\end{center}
\end{figure}



% the extent to which the game between the two principals is competitive
% degree of innovation that these models incentivize.
% the extent to which agents make rational decisions


%\subsection{Our model}
%\label{sec:intro-model}

\xhdr{Our model.} We define a game in which two firms (\emph{principals}) simultaneously engage in exploration and compete for users (\emph{agents}). These two processes are interlinked, as exploration decisions are experienced by users and informed by their feedback. We need to specify several conceptual pieces: how the principals and agents interact, what is the machine learning problem faced by each principal, and what is the information structure. Each piece can get rather complicated in isolation, let alone jointly, so we strive for simplicity. Thus, the basic model is as follows:

\begin{itemize}

\item A new agent arrives in each round $t=1,2, \ldots$, and chooses among the two principals. The principal chooses an action (\eg a list of web search results to show to the agent), the user experiences this action, and reports a reward. \asedit{All agents have the same ``decision rule" for choosing among the principals given the available information.}

\item Each principal faces a very basic and well-studied version of the multi-armed bandit problem: for each arriving agent, it chooses from a fixed set of actions  (a.k.a. \emph{arms}) and receives a reward drawn independently from a fixed distribution specific to this action.

\item Principals simultaneously announce their learning algorithms \asedit{before round $1$}, and cannot change them afterwards. There is a common Bayesian prior on the rewards (but the realized reward distributions are not observed by the principals or the agents). Agents do not receive \asedit{any other information}. Each principal only observes agents that chose him.
\end{itemize}

\xhdr{Technical results.}
Our results depend crucially on agents' ``decision rule" for choosing among the principals. The simplest and perhaps the most obvious rule is to select the principal which maximizes their expected utility; we refer to it as \HardMax. We find that \HardMax is not conducive to \asedit{adopting better algorithms}. In fact, each principal's dominant strategy is to do no purposeful exploration whatsoever, and instead always choose an action that maximizes expected reward given the current information; we call this algorithm \DynGreedy. While this algorithm may potentially try out different actions over time and acquire useful information, it is known to be dramatically bad in many important cases of multi-armed bandits --- precisely because it does not explore on purpose, and may therefore fail to discover best/better actions. Further, we show that \HardMax is very sensitive to tie-breaking when both principals have exactly the same expected utility according to agents' beliefs. If tie-breaking is probabilistically biased --- say, principal 1 is always chosen with probability strictly larger than $\tfrac12$ --- then this principal has a simple ``winning strategy" no matter what the other principal does.

We relax \HardMax to allow each principal to be chosen with some fixed baseline probability. One intuitive interpretation is that there are ``random agents" who choose a principal uniformly at random, and each arriving agent is either \HardMax or ``random" with some fixed probability. We call this model \HardMaxRandom. We find that \asedit{better algorithms} help in a big way: a sufficiently better algorithm is guaranteed to win all \asedit{non-random} agents after an initial learning phase. While the precise notion of ``sufficiently better algorithm" is rather subtle, we note that commonly known ``smart" bandit algorithms typically defeat the commonly known ``naive" ones, and the latter typically defeat \DynGreedy. However, there is a substantial caveat: one can defeat any algorithm by interleaving it with \DynGreedy. This has two undesirable corollaries: a better algorithm may sometimes lose, and a pure Nash equilibrium typically does not exist.

We further relax the decision rule so that the probability of choosing a given principal varies smoothly as a function of the difference between  principals' expected rewards; we call it \SoftMaxRandom. For this model, the ``better algorithm wins" result holds under much weaker assumptions on what constitutes a better algorithm. This is the most technical result of the paper. The competition in this setting is necessarily much more relaxed: typically, both principals attract approximately half of the agents as time goes by (but a better algorithm may attract slightly more).

All results extend to a much more general version of the multi-armed bandit problem in which the principal may observe additional feedback before and/or after each decision, as long as the feedback distribution does not change over time. In most results, principal's utility may depend on both the market share and agents' rewards.

\xhdr{Economic interpretation.}
\asedit{The inverted-U relationship between the severity of competition among firms and the quality of technologies that they adopt is a familiar theme in the economics literature \citep[\eg][]{Aghion-QJE05,Vives-08}.%
\footnote{The literature frames this relationship as one between ``competition" and ``innovation". In this context, ``innovation" refers to adoption of a better technology, at a substantial R\&D expense to a given firm. It is not salient whether similar ideas and/or technologies already exist outside the firm. It is worth noting that adoption of exploration algorithms tends to require substantial R\&D effort in practice, even if the algorithms themselves are well-known in the research literature; see \citet{MWT-WhitePaper-2016} for an example of such R\&D effort.}
We find it illuminating to frame our contributions in a similar manner, as illustrated in \reffig{fig:inverted-U}.

Our models differ in terms of rationality in agents' decision-making: from fully rational decisions with \HardMax to relaxed rationality with \HardMaxRandom to an even more relaxed rationality with \SoftMaxRandom. The same distinctions also control the severity of competition between the principals: from cut-throat competition with \HardMax to a more relaxed competition with \HardMaxRandom, to an even more relaxed competition with \SoftMaxRandom. Indeed, with \HardMax you lose all customers as soon as you fall behind in performance, with \HardMaxRandom you get some small market share no matter what, and with \SoftMaxRandom you are further guaranteed a market share close to $\tfrac12$ as long as your performance is not much worse than the competition. The uniform choice among principals corresponds to no rationality and no competition.

We identify the inverted-U relationship in the spirit of \reffig{fig:inverted-U} that is driven by the rationality/competitiveness distinctions outlined above: from \HardMax to \HardMaxRandom to \SoftMaxRandom to \Uniform. We also find another, technically different inverted-U relationship which zeroes in on the \HardMaxRandom model. We vary rationality/competitiveness inside this model, and track the marginal utility of switching to a better algorithm.

These inverted-U relationships arise for a fundamentally different reason, compared to the existing literature on ``competition vs. innovation.'' In the literature, better technology always helps in a competitive environment, other things being equal. Thus, the tradeoff is between the costs of improving the technology and the benefits that the improved technology provides in the competition. Meanwhile, we find that a better exploration algorithm may sometimes perform much worse under competition, even in the absence of R\&D costs.}

\ascomment{Yishay's edits, slightly edited by Alex}

\xhdr{Discussion.} We capture some pertinent features of reality while ignoring some others for the sake of tractability. Most notably, we assume that agents do not receive any information about other agents' rewards after the game starts. In the final analysis, this assumption makes agents' behavior independent of a particular realization of the Bayesian prior, and therefore enables us to summarize each learning algorithm via its Bayesian-expected rewards (as opposed to detailed performance on the particular realizations of the prior). Such summarization is essential for formulating lucid and general analytic results, let alone proving them. It is a major open question whether one can incorporate signals about other agents' rewards and obtain a tractable model.

We also make a standard assumption that agents are myopic: they do not worry about how their actions impact their future utility. In particular, they do not attempt to learn over time, to second-guess or game future agents, or to manipulate principal's learning algorithm. We believe this is a typical case in practice, in part because agent's influence tend to be small compared to the overall system. We model this simply by assuming that each agent only arrives once.

Much of the challenge in this paper, both conceptual and technical, was in setting up the right model and the matching theorems, and not only in proving the theorems. Apart from making the modeling choices described above, it was crucial to interpret the results and intuitions from the literature on multi-armed bandits so as to formulate meaningful assumptions on bandit algorithms and Bayesian priors which are productive in our setting.

\xhdr{Open questions.}
\asedit{How to incorporate signals about the other agents' rewards? One needs to reason about how exact or coarse these signals are, and how the agents update their beliefs after receiving them. Also, one may need to allow principals' learning algorithms to respond to updates about the other principal's performance. (Or not, since this is not how learning algorithms are usually designed!) A clean, albeit idealized, model would be that (i) each agent learns her exact expected reward from each principal before she needs to choose which principal to go to, but (ii) these updates are invisible to the principals. Even then, one needs to argue about the competition on particular realizations of the Bayesian prior, which appears very challenging.

Another promising extension is to heterogeneous agents. Then the agents' choices are impacted by their idiosyncratic signals/beliefs, instead of being entirely determined by priors and/or signals about the average performance. It would be particularly interesting to investigate the emergence of \emph{specialization}: whether/when an algorithm learns to target specific population segments in order to compete against a more powerful ``incumbent".
} %\asedit


\xhdr{Map of the paper.}
We survey related work (Section~\ref{sec:related-work}), lay out the model and preliminaries (Section~\ref{sec:model}), and proceed to analyze the three main models, \HardMax, \HardMaxRandom and \SoftMaxRandom (in Sections~\ref{sec:rational},~\ref{sec:random}, and ~\ref{sec:soft}, respectively). We discuss economic implications in Section~\ref{sec:welfare}. Appendix~\ref{app:examples} provides some pertinent background on multi-armed bandits. Appendix~\ref{app:perturb} gives a broad example to support an  assumption in our model.




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> itcs18paper/sec-random.tex <==
This section is dedicated to the \HardMaxRandom response model, where each principal is always chosen with some positive baseline probability. The main technical result for this model states that a principal with asymptotically better \BIR wins by a large margin: after a ``learning phase" of constant duration, all agents choose this principal with maximal possible probability $\respF(1)$. For example, a principal with $\BIR(n)\leq \tilde{O}(n^{-1/2})$ wins over a principal with $\BIR(n)\geq \Omega(n^{-1/3})$. However, this positive result comes with a significant caveat detailed in Section~\ref{sec:random-greedy}.

We formulate and prove a cleaner version of the result, followed by a more general formulation developed in a subsequent Remark~\ref{rem:random-messy}. We need to express a property that \alg[1] eventually catches up and surpasses \alg[2], even if initially it receives only a fraction of traffic. For the cleaner version, we assume that both algorithms are well-defined for an infinite time horizon, so that their \BIR does not depend on the time horizon $T$ of the game.  Then this property can be formalized as:
\begin{align}\label{eq:random-better-clean}
(\forall \eps>0)\qquad
\BIR_1(\eps n)/\BIR_2(n) \to 0.
\end{align}
In fact, a weaker version of \eqref{eq:random-better-clean} suffices:
denoting $\eps_0 = \respF(-1)$, for some constant $n_0$ we have
\begin{align}\label{eq:random-better-weaker}
(\forall n\geq n_0) \qquad
\BIR_1(\eps_0 n/2)/\BIR_2(n) <\tfrac12.
\end{align}
We also need a very mild technical assumption on the ``bad" algorithm:
\begin{align}\label{eq:random-assn}
 (\forall n\geq n_0) \qquad
  \BIR_2(n) > 4\,e^{-\eps_0 n/12}.
\end{align}

\begin{theorem}\label{thm:random-clean}
Assume \HardMaxRandom response function. Suppose both algorithms are monotone and well-defined for an infinite time horizon, and satisfy~\eqref{eq:random-better-weaker} and~\eqref{eq:random-assn}. Then each agent $t\geq n_0$ chooses principal $1$ with maximal possible probability $\respF(1) = 1- \eps_0$.
\end{theorem}

\begin{proof}
Consider global round $t\geq n_0$. Recall that each agent chooses principal $1$ with probability at least
    $\respF(-1)>0$.

Then
    $\E[n_1(t+1)] \geq 2\eps_0\,t $.
By Chernoff Bounds (Theorem~\ref{thm:chernoff}), we have that
    $n_1(t+1)\geq \eps_0 t$
holds with probability at least $1-q$,
where $q = \exp(-\eps_0 t/12)$.

We need to prove that
    $\PMR_1(t) - \PMR_2(t)>0$.
For any $m_1$ and $m_2$, consider the quantity
\[ \Delta(m_1,m_2) := \BIR_2(m_2+1) - \BIR_1(m_1+1).\]
Whenever $m_1 \geq \eps_0 t/2 -1$ and $m_2<t$, it holds that
\begin{align*}
\Delta(m_1,m_2) \geq \Delta(\eps_0 t / 2, t)
    \geq \BIR_2(t)/2.
\end{align*}
The above inequalities follow, resp., from algorithms' monotonicity and \eqref{eq:random-better-weaker}. Now,
\begin{align*}
\PMR_1(t) - \PMR_2(t)
    &= \Ex{m_1\sim \posteriorN{1}{t},\;m_2\sim \posteriorN{2}{t}}{\Delta(m_1,m_2)} \\
    &\geq -q
        + \Ex{m_1\sim \posteriorN{1}{t},\;m_2\sim \posteriorN{2}{t}}
            {\Delta(m_1,m_2)\mid m_1 \geq \eps_0 t/2-1} \\
    &\geq \BIR_2(t)/2-q \\
    &> \BIR_2(t)/4 > 0  \EqComment{by \eqref{eq:random-assn}}. \qedhere
\end{align*}
\end{proof}

\begin{remark}\label{rem:random-messy}
  Many standard MAB algorithms in the literature are parameterized by
  the time horizon $T$. Regret bounds for such algorithms usually
  include a polylogarithmic dependence on $T$. In particular, a
  typical upper bound for \BIR has the following form:
  \OMIT{\footnote{We
    provide upper bounds on \BIR for several standard MAB algorithms
    to illustrate these dependencies in the appendix.\sw{added}}}
\begin{align}
    \BIR(n\mid T)\leq \polylog(T)\cdot n^{-\gamma}
    \quad \text{for some $\gamma\in(0,\tfrac12]$}.
\end{align}
Here we write $\BIR(n\mid T)$ to emphasize the dependence on $T$.

We generalize \eqref{eq:random-better-weaker} to handle the dependence
on $T$: there exists a number $T_0$ and a function $n_0(T)\in \polylog(T)$ 
such that 
\begin{align}\label{eq:random-better-messy}
(\forall T\geq T_0,\; n\geq n_0(T)) \quad
\frac{\BIR_1(\eps_0 n /2\mid T)}{\BIR_2(n\mid T)} <\frac12.
\end{align}
If this holds, we say that \alg[1] \emph{BIR-dominates} \alg[2].

We provide a version of Theorem~\ref{thm:random-clean} in which algorithms are parameterized with time horizon $T$ and condition \eqref{eq:random-better-weaker} is replaced with \eqref{eq:random-better-messy}; its proof is very similar and is omitted.
\end{remark}

%\begin{theorem}\label{thm:random-messy}
%Assume \HardMaxRandom response function, and algorithms that satisfy \eqref{eq:random-better-messy} and~\eqref{eq:random-assn}. Then each agent
%    $t\geq n_0(T)$ chooses principal $1$ with probability $\respF(1)$.
%\end{theorem}


%Let \alg be a monotone MAB algorithm and $\mA$ be a finite set of monotone MAB algorithms such that each algorithm in $\mA$ satisfies \eqref{eq:random-assn} and is ``dominated" by \alg in the sense of \eqref{eq:random-better-messy}.
%Assume principals can only choose algorithms from $\mA\cup \{\alg\}$.

To state a game-theoretic corollary of Theorem~\ref{thm:random-clean}, we consider a version of the competition game between the two principals in which they can only choose from a finite set $\mA$ of monotone MAB algorithms. One of these algorithms is ``better" than all others; we call it the \emph{special} algorithm. Unless specified otherwise, it BIR-dominates all other allowed algorithms. The other algorithms satisfy \eqref{eq:random-assn}. We call this game the \emph{restricted competition game}.

\begin{corollary}\label{cor:random}
Assume \HardMaxRandom response function. Consider the restricted competition game with special algorithm \alg. Then, for any sufficiently large time horizon $T$, this game has a unique Nash equilibrium: both principals choose \alg.
\end{corollary}


\subsection{A little greedy goes a long way}
\label{sec:random-greedy}

Given any monotone MAB algorithm other than \DynGreedy, we design a modified algorithm which learns at a slower rate, yet ``wins the game" in the sense of Theorem~\ref{thm:random-clean}. As a corollary, the competition game with unrestricted choice of algorithms typically does not have a Nash equilibrium.

Given an algorithm \alg[1] that deviates from \DynGreedy starting from
step $n_0$ and a ``mixing'' parameter $p$, we will construct a
modified algorithm as follows.
\begin{enumerate}
\item The modified algorithm coincides with \alg[1] (and \DynGreedy)
for the first $n_0-1$ steps;
\item In each step $n\geq n_0$, \alg[1] is invoked with probability
  $1-p$, and with the remaining probability $p$ does the ``greedy
  choice": chooses an action with the largest posterior mean reward
  given the current information collected by \alg[1].
\end{enumerate}
%The modified algorithm is called \emph{greedy deviation}, with probability parameter $p$.
For a cleaner comparison between the two algorithms, the modified algorithm does not record rewards received in steps with the ``greedy choice". Parameter $p>0$ is the same for all steps. We state the main result and defer the detailed proof to the appendix.

\begin{theorem}\label{thm:random-greedy}
Assume symmetric \HardMaxRandom response function. Let $\eps_0 = \respF(-1)$ be the baseline probability. Suppose \alg[1] deviates from \DynGreedy starting from some step $n_0$. Let \alg[2] be the modified algorithm, as described above, with mixing parameter $p$ such that
    $(1-\eps_0)(1-p)>\eps_0$.
Then each agent $t\geq n_0$ chooses principal $2$ with maximal possible probability $1-\eps_0$.
\end{theorem}

\begin{corollary}\label{cor:random-greedy}
  Suppose that both principals can choose any monotone MAB algorithm, and assume the symmetric \HardMaxRandom response
  function. Then for any time
  horizon $T$, the only possible \emph{pure} Nash equilibrium is one
  where both principals choose \DynGreedy. Moreover, no pure Nash
  equilibrium exists when some algorithm ``dominates" \DynGreedy in
  the sense of \eqref{eq:random-better-messy} and the time horizon $T$
  is sufficiently large.
\end{corollary}


\begin{remark}
The modified algorithm performs exploration % ingests information
at a slower rate. Let us argue how this may translate  into a larger \BIR compared to the original algorithm. Let  $\BIR'_1(n)$ be the \BIR of the ``greedy choice" after after $n-1$ steps of \alg[1]. Then
\begin{align}\label{eq:random-BIR}
\BIR_2(n)
    &= \Ex{m\sim (n_0-1)+\term{Binomial}(n-n_0+1,1-p)}{(1-p) \cdot \BIR_1(m) + p \cdot \BIR'_1(m)}.
\end{align}
In this expression, $m$ is the number of times \alg[1] is invoked in the first $n$ steps of the modified algorithm. Note that
    $\E[m] = n_0-1 + (n-n_0+1)(1-p) \geq (1-p)n$.

Suppose $\BIR_1(n)= \beta n^{-\gamma}$ for some constants $\beta,\gamma>0$. Further, assume 
    $\BIR'_1(n)\geq  c\; \BIR_1(n)$,
for some $c>1-\gamma$.
Then for all $n\geq n_0$ and small enough $p>0$ it holds that:
\begin{align*}
 \BIR_2(n) 
    &\geq  (1-p+pc)\; \E[\; \BIR_1(m) \;] \\
\E[\; \BIR_1(m) \;]
    &\geq \BIR_1(\; \E[m] \;) &\qquad\text{(By Jensen's inequality)} \\
    &\geq \BIR_1(\; (1-p)n \;) &\qquad\text{(since $\E[m]\geq n(1-p)$)}  \\
    &\geq \beta\cdot n^{-\gamma} \cdot (1-p)^{-\gamma} 
        &\qquad\text{(plugging in $\BIR_1(n)=\beta n^{-\gamma}$)}  \\
    &> \BIR_1(n)\;\; (1-p\gamma)^{-1}
        &\qquad\text{(since $(1-p)^\gamma < 1-p\gamma$)}.\\
\BIR_2(n) 
    &>\alpha\cdot \BIR_1(n),
    &\text{where} \quad 
    \alpha = \tfrac{1-p+pc}{1-p\gamma}>1.
\end{align*}
(In the above equations, all expectations are over $m$ distributed as in \eqref{eq:random-BIR}.)
\end{remark}

%%% Local Variables:
%%% TeX-master: "main.tex"
%%% End: 

==> itcs18paper/sec-rational.tex <==

In this section, we will consider the version in which
the agents are fully rational, in the sense that their response function is \HardMax. We show that principals are not incentivized to \emph{explore}--- \ie to deviate from \DynGreedy. The core technical result is that if one principal adopts \DynGreedy, then the other principal loses all agents as soon as he deviates.

To make this more precise, let us say that two MAB algorithms \emph{deviate} at (local) step $n$ if there is an action $a\in A$ and \asedit{a set of step-$n$ histories of positive probability such that any history $h$ in this set} is feasible for both algorithms, and under this history the two algorithms choose action $a$ with different probability.

\iffalse
\begin{definition}
  Suppose that an algorithm $\pi$ is not dynamic greedy. Then
  {\em the first exploration} for $\pi$ is the first time step where
  there is a non-zero probability that the recommended action has a
  lower expectation than exploitation option.\sw{define...}
\end{definition}
\fi


\begin{theorem}\label{thm:DG-dominance}
Assume \HardMax response function with fair tie-breaking. Assume that \alg[1] is \DynGreedy, and \alg[2] deviates from \DynGreedy starting from some (local) step $n_0<T$. Then all agents in global rounds $t\geq n_0$ select principal $1$.
\end{theorem}

\begin{corollary}\label{cor:DG-dominance}
The competition game between principals has a unique Nash equilibirium: both principals choose \DynGreedy.
\end{corollary}


\begin{remark}
This corollary holds under a more general model which allows time-discounting: namely, the utility of each principal $i$ in each global round $t$ is $U_{i,t}(r_t)$ if this principal is chosen, and $0$ otherwise, where $U_{i,t}(\cdot)$ is an arbitrary non-decreasing function with $U_{i,t}(0)>0$.
\end{remark}

\subsection{Proof of Theorem~\ref{thm:DG-dominance}}

The proof starts with two auxiliary lemmas: that deviating from \DynGreedy implies a strictly smaller Bayesian-expected reward, and that \HardMax implies a ``sudden-death" property: if one agent chooses principal $1$ with certainty, then so do all subsequent agents do. \asedit{We re-use both lemmas in later sections, so we state them in sufficient generality.}


\begin{lemma}\label{lm:DG-rew}
\asedit{Assume that \alg[1] is \DynGreedy, and \alg[2] deviates from \DynGreedy starting from some (local) step $n_0<T$. Then $\rew_1(n_0)>\rew_2(n_0)$. This holds for any response function $\respF$.}
\end{lemma}

\asedit{Lemma~\ref{lm:DG-rew} does not rely on any particular shape of the response function because it only considers the performance of each algorithm without competition.}

\begin{proof}[Proof of Lemma~\ref{lm:DG-rew}]
Since the two algorithms coincide on the first $n_0-1$ steps, it follows by symmetry that histories $H_{1,n_0}$ and $H_{2,n_0}$ have the same distribution. We use a \emph{coupling argument}: w.l.o.g., we assume the two histories coincide,
    $H_{1,n_0} = H_{2,n_0} = H$.

At local step $n_0$, \DynGreedy chooses an action $a_{1,n_0} = a_{1,n_0}(H)$
which maximizes the posterior mean reward given history $H$: for any realized history $h\in \support(H)$ and any action $a\in A$
\begin{align}\label{eq:lm:DG-rew-1}
 \PMR(a_{1,n_0} \mid H = h) \geq \PMR(a \mid H=h).
\end{align}

\ascomment{Rewrote the rest of the proof to account for positive-prob set of histories.}

By assumption \eqref{eq:assn-distinct}, it follows that 
\begin{align}\label{eq:lm:DG-rew-2}
 \PMR(a_{1,n_0} \mid H = h) > \PMR(a \mid H=h)
 \quad \text{for any $h\in \support(H)$ and $a\neq a_{1,n_0}(h)$.}
\end{align}

Since the two algorithms deviate at step $n_0$, there is a set $S\subset \support(H)$ of step-$n_0$ histories such that $\Pr[S]>0$ and any history $h\in S$ satisfies
    $\Pr[a_{2,n_0}\neq a_{1,n_0} \mid H=h]>0$.
Combining this with \eqref{eq:lm:DG-rew-2}, we deduce that 
\begin{align}\label{eq:lm:DG-rew-3}
 \PMR(a_{1,n_0} \mid H = h) > \E\left[ \mu_{a_{2,n_0}}\mid H=h \right]
 \quad\text{for each history $h\in S$}.
\end{align}
Using \eqref{eq:lm:DG-rew-1} and \eqref{eq:lm:DG-rew-3} and integrating over realized histories $h$, we obtain
    $\rew_1(n_0) > \rew_2(n_0)$.
\end{proof}


\begin{lemma}\label{lm:DG-sudden}
\asedit{Consider \HardMax response function with $\respF(0)\geq\tfrac12$.} 
Suppose \alg[1] is monotone, and $\PMR_1(t_0)>\PMR_2(t_0)$ for some global round $t_0$. Then $\PMR_1(t)>\PMR_2(t)$ for all subsequent rounds $t$.
\end{lemma}

\begin{proof}
Let us use induction on round $t\geq t_0$, with the base case $t=t_0$. Let $\mN=\mN_{1,t_0}$ be the agents' posterior distribution for $n_{1,t_0}$, the number of global rounds before $t_0$ in which principal $1$ is chosen. By induction, all agents from $t_0$ to $t-1$ chose principal $1$, so $\PMR_2(t_0)= \PMR_2(t)$. Therefore,
\[ \PMR_1(t)
    = \Ex{n\sim \mN}{\rew_1(n+1+t-t_0)}
    \geq \Ex{n\sim \mN}{\rew_1(n+1)}
    =\PMR_1(t_0) > \PMR_2(t_0)= \PMR_2(t), \]
where the first inequality holds because \alg[1] is monotone, and the second one is the base case.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:DG-dominance}]
Since the two algorithms coincide on the first $n_0-1$ steps, it follows by symmetry that $\rew_1(n) = \rew_2(n)$ for any $n< n_0$.
By Lemma~\ref{lm:DG-rew},
    $\rew_1(n_0) > \rew_2(n_0)$.

Recall that $n_i(t)$ is the number of global rounds $s<t$ in which principal $i$ is chosen, and $\posteriorN{i}{t}$ is the agents' posterior distribution for this quantity. By symmetry, each agent $t<n_0$ chooses a principal uniformly at random. It follows that
    $\posteriorN{1}{n_0} = \posteriorN{2}{n_0}$
(denote both distributions by $\mN$ for brevity), and $\mN(n_0-1)>0$.
Therefore:
\begin{align}
\PMR_1(n_0)
  &= \Ex{n\sim \mN} {\rew_1(n+ 1)}
   = \sum_{n = 0}^{n_0-1} \mN(n) \cdot{\rew_1(n + 1)} \nonumber \\
  & > \mN(n_0-1)\cdot {\rew_2(n_0)} + \sum_{n = 0}^{n_0-2}  \mN(n)\cdot{\rew_2(n + 1)}
    \nonumber \\
  &= \Ex{n\sim \mN}{\rew_2(n + 1)} = \PMR_2(n_0) \label{eq:pf:thm:DG-dominance}
\end{align}
So, agent $n_0$ chooses principal $1$. By Lemma~\ref{lm:DG-sudden} \asedit{(noting that \DynGreedy is monotone)}, all subsequent agents choose principal $1$, too.
\end{proof}


%\begin{theorem}
%  Suppose that the agents break ties uniformly at random, that is
%  $q=1/2$, then both principals playing \DynGreedy is the unique
%  equilibrium.
%\end{theorem}
%
%\begin{proof}
%  Suppose that both principals play dynamic greedy. The result
%  of Theorem~\ref{thm:DG-dominance} shows that there is no beneficial deviation
%  for both principals, so this forms a pure strategy equilibrium.
%
%  Now we will show that no other strategy profile can form equilibrium
%  in this game.  Suppose that both principals play some mixed
%  strategies that places non-zero probability on algorithms other than
%  dynamic greedy. We know one of the principals $p_j$ is getting no
%  more than $T/2$ agents in expectation. If $p_j$ switch to playing
%  only dynamic greedy, he can get strictly more than $T/2$ agents
%  by Theorem~\ref{thm:DG-dominance}. Thus, such a strategy profile will not form
%  an equilibrium.  Finally, suppose that $p_1$ plays dynamic greedy
%  and $p_2$ plays algorithms other than dynamic greedy with non-zero
%  probability. By Theorem~\ref{thm:DG-dominance}, we know that $p_2$ gets less
%  than $T/2$ agents in expectation. This means switching to dynamic
%  greedy will strictly improve the expected utility to $T/2$, so such
%  strategy profile cannot form an equilibrium either.
%\end{proof}


\subsection{\HardMax with biased tie-breaking}
\label{sec:HardMax-biased}

The \HardMax model is very sensitive to the tie-breaking rule. For starters, if ties are  broken deterministically in favor of principal $1$, then principal 1 can get all agents no matter what the other principal does, simply by using \StaticGreedy.

\begin{theorem}\label{thm:HardMax-hardTies}
Assume \HardMax response function with $\respF(0)=1$ (ties are always broken in favor of principal $1$). If \alg[1] is \StaticGreedy, then all agents choose principal $1$.
\end{theorem}

\begin{proof}
Agent $1$ chooses principal $1$ because of the tie-breaking rule. Since \StaticGreedy is trivially monotone, all the subsequent agents choose principal $1$ by an induction argument similar to the one in the proof of Lemma~\ref{lm:DG-sudden}.
\end{proof}

A more challenging scenario is when the tie-breaking is biased in favor of principal 1, but not deterministically so: $\respF(0)>\tfrac12$. Then this principal also has a ``winning strategy" no matter what the other principal does. Specifically, principal 1 can get all but the first few agents, under a mild technical assumption that \DynGreedy deviates from \StaticGreedy. Principal 1 can use \DynGreedy, or any other monotone MAB algorithm that coincides with \DynGreedy in the first few steps. We state the result and defer the proof to the appendix.

%We can generalize the theorem top the case of $q >1/2$ if the
%principal $p_1$ can guarantee better than the a priori best action to
%all the agents following the second.


\begin{theorem}\label{thm:HardMax-biased}
Assume \HardMax response function with $\respF(0)>\tfrac12$ (\ie tie-breaking is biased in favor of principal $1$). Assume the prior $\mP$ is such that \DynGreedy deviates from \StaticGreedy starting from some step $n_0$. Suppose that principal $1$ runs a monotone MAB algorithm that coincides with \DynGreedy in the first $n_0$ steps. Then all agents $t\geq n_0$ choose principal $1$.
\end{theorem}


% OLD PROOF (assuming alg1 coincides with DG on first two rounds, etc.
% We consider two cases, depending on the arm $a_{2,1}$ that principal $2$ chooses in the same step. The interesting case is $a_{2,1}=1$.
%Then agent $1$ selects principal $1$ with probability $q:=\respF(0)>\tfrac12$. Therefore, agent $2$ forms the following posterior mean rewards:
%\begin{align*}
%  \PMR_1(2) &= (1-q)\cdot \E[\mu_1] + q\cdot \rew_1(2)
%    \EqComment{for principal 1}\\
%  \PMR_2(2) &= q\cdot \E[\mu_1] + (1-q)\cdot \rew_2(2)
%    \EqComment{for principal 2}.
%\end{align*}
%We know that
%    $\rew_1(2) > \E[\mu_1]$
%(\DynGreedy is strictly monotone in the first $2$ rounds)
%from Lemma~\ref{dgmono}, and
%    $\rew_1(2) \geq \rew_2(2)$
%by Lemma~\ref{lm:DG-rew}. It follows that
%    $\PMR_1(2)>\PMR_2(2)$,
%and consequently agent $2$ chooses principal $1$. The subsequent agents choose principal $1$ by Lemma~\ref{lm:DG-sudden}.
%
%The remaining case is $a_{2,1}\neq 1$: principal $p_2$ does not recommend arm $1$ in the first step. Since all other arms have a strictly lower prior mean reward, agent $1$ chooses principal $1$. The subsequent agents choose principal $1$ by Lemma~\ref{lm:DG-sudden}.



% \begin{lemma}
%   Let $\mu^2_{DG}$ the expected reward of action of \DynGreedy
%   in the second step. Then $\mu^2_{DG} > \mu_1$.
% \end{lemma}

% \begin{proof}
%   \sw{todo. This requires an assumption that the second arm has
%     non-zero probability of beating the first one.}
% \end{proof}



% Steven's proof for a more general version with alg1 = BIC algo
%Agent $1$ chooses principal $1$ because of the tie-breaking rule,
%  Since principal $p_1$ in the first step recommends arm 1, the agent
%  selects principal $p_1$ (due to the tie breaking rule).  Agent $2$
%  knows that agent $1$ selected $p_1$. Because of BIC, she knows $p_1$
%  will offer reward no lower than $p_2$ in expectation.  By induction,
%  all the agents select principal $p_1$.



%\sw{We also have an observation saying if one principal starts with a
%  better dynamic greedy will just dominate the game. It could do some
%  amount of exploration while having better Bayesian per-round regret
%  than the other principal. This means the other principal will never
%  have any agents arriving for learning.}

%%% Local Variables:
%%% TeX-master: "main.tex"
%%% End: 

==> itcs18paper/sec-related-work.tex <==
Multi-armed bandits (\emph{MAB}) is a particularly elegant and tractable abstraction for tradeoff between \emph{exploration} and \emph{exploitation}: essentially, between acquisition and usage of information. MAB problems have been studied in Economics, Operations Research and Computer Science for many decades; see \citep{Bubeck-survey12,Gittins-book11,slivkins-MABbook} for background on regret-minimizing and Bayesian formulations, respectively. A discussion of industrial applications of MAB can be found in \citet{MWT-WhitePaper-2016}.

The literature on MAB is vast and multi-threaded. The most related
thread concerns regret-minimizing MAB formulations with IID rewards
\citep{Lai-Robbins-85,bandits-ucb1}. This thread includes ``smart" MAB
algorithms that combine exploration and exploitation, such as UCB1
\citep{bandits-ucb1} and Successive Elimination
\citep{EvenDar-icml06}, and ``naive'' MAB algorithms that separate
exploration and exploitation, including explore-first and
$\eps$-Greedy \citep[\eg see][]{slivkins-MABbook}.

The three-way tradeoff between exploration, exploitation and incentives has been studied in several other settings:
incentivizing exploration in a recommendation system
    \citep{Che-13,Frazier-ec14,Kremer-JPE14,ICexploration-ec15,Bimpikis-exploration-ms17,Bahar-ec16,ICexplorationGames-ec16-working},
dynamic auctions
    \cite[\eg][]{AtheySegal-econometrica13,DynPivot-econometrica10,Kakade-pivot-or13},
pay-per-click ad auctions with unknown click probabilities
    \cite[\eg][]{MechMAB-ec09,DevanurK09,Transform-ec10-jacm},
coordinating search and matching by self-interested agents
    \citep{Bobby-Glen-ec16},
as well as human computation
    \cite[\eg][]{RepeatedPA-ec14,Ghosh-itcs13,Krause-www13}.

\citet{Bolton-econometrica99,Keller-econometrica05,Johari-ec12} studied models with self-interested agents jointly performing exploration, with no principal to coordinate them.

There is a superficial similarity (in name only) between this paper and the line of work on ``dueling bandits"
    \citep[\eg][]{Yue-dueling12,Yue-dueling-icml09}.
The latter is not about competing bandit algorithms, but rather about scenarios where in each round two arms are chosen to be presented to a user, and the algorithm only observes which arm has ``won the duel".

Our setting is closely related to the ``dueling algorithms" framework \citep{DuelingAlgs-stoc11} which studies competition between two principals, each running an algorithm for the same problem. However, this work considers algorithms for offline / full input scenarios, whereas we focus on online machine learning and the explore-exploit-incentives tradeoff therein. Also, this work specifically assumes binary payoffs (\ie win or lose) for the principals.

\xhdr{Other related work in economics.} The competition vs. innovation relationship and the inverted-U shape thereof have been introduced in a classic book \citep{Schumpeter-42}, and remained an important theme in the literature ever since \cite[\eg][]{Aghion-QJE05,Vives-08}. Production costs aside, this literature treats innovation as a priori beneficial for the firm. Our setting is very different, as innovation in exploration algorithms may potentially hurt the firm.

A line of work on \emph{platform competition}, starting with \cite{Rysman09}, concerns competition between firms (\emph{platforms}) that improve as they attract more users (\emph{network effect}); see \citet{Weyl-White-14} for a recent survey. This literature is not concerned with \innovation, and typically models network effects exogenously, whereas in our model network effects are endogenous: they are created by MAB algorithms, an essential part of the model.

Relaxed versions of rationality similar to ours are found in several notable lines of work. For example, ``random agents" (a.k.a. noise traders) can side-step the ``no-trade theorem'' \citep{Milgrom-Stokey-82}, a famous impossibility result in financial economics. The \SoftMaxRandom model is closely related to the literature on \emph{product differentiation}, starting from \cite{Hotelling-29}, see \cite{Perloff-Salop-85} for a notable later paper.

There is a large literature on non-existence of equilibria due to small deviations   (which is related to the corresponding result for \HardMaxRandom), starting with \cite{Rothschild-Stiglitz-76} in the context of health insurance markets. Notable recent papers \citep{Veiga-Weyl-16,Azevedo-Gottlieb-17} emphasize the distinction between \HardMax and versions of \SoftMaxRandom.

% moved this thought to the intro.
\OMIT{While agents' rationality and severity of competition are often modeled separately in the literature, it is not unusual to have them modeled with the same ``knob" \cite[\eg][]{Gabaix-16}.}





%%% Local Variables:
%%% TeX-master: "main.tex"
%%% End: 

==> itcs18paper/sec-soft.tex <==
This section is devoted to the \SoftMaxRandom model. We recover a positive result under the assumptions from Theorem~\ref{thm:random-clean} (albeit with a weaker conclusion), and then proceed to a much more challenging result under weaker assumptions. We start with a formal definition:

\begin{definition}\label{def:SoftMax}
A response function $\respF$ is \SoftMaxRandom if the following conditions hold:
\begin{OneLiners}
\item  $\respF(\cdot)$ is bounded away from $0$ and $1$:
    $\respF(\cdot)\in [\eps,1-\eps]$ for some $\eps\in (0,\tfrac12)$,
\item  the response function
 $\respF(\cdot)$ is ``smooth" around $0$:
 \begin{align}\label{eq:SoftMax-smooth}
 \exists\, \text{constants $\delta_0,c_0,c'_0>0$}
    \qquad \forall x\in [-\delta_0,\delta_0] \qquad
    c_0 \leq \respF'(x) \leq c'_0.
 \end{align}
\item fair tie-breaking: $\respF(0)=\tfrac12$.
\end{OneLiners}
\end{definition}

\begin{remark}
\asedit{This definition is fruitful when parameters $c_0$ and $c_0'$ are close to $\tfrac12$. Throughout, we assume that \alg[1] is better than \alg[2], and obtain results parameterized by $c_0$. By symmetry, one could assume that \alg[2] is better than \alg[1], and obtain similar results parameterized by $c_0'$.}
\end{remark}

Our first result is a version of Theorem~\ref{thm:random-clean}, with the same assumptions about the algorithms and essentially the same proof. The conclusion is much weaker: we can only guarantee that each agent $t\geq n_0$ chooses principal 1 with probability slightly larger than $\tfrac12$. This is essentially unavoidable in a typical case when both algorithms satisfy $\BIR(n)\to 0$, by Definition~\ref{def:SoftMax}.

\begin{theorem}\label{thm:SoftMax-weak}
  Assume \SoftMaxRandom response function. Suppose \alg[1] has better
  \BIR in the sense of \eqref{eq:random-better-weaker}, and \alg[2]
  satisfies the condition \eqref{eq:random-assn}. Then each agent
  $t\geq n_0$ chooses principal $1$ with probability
\begin{align}\label{eq:thm:SoftMax-weak}
     \Pr[i_t = 1]\geq \tfrac12 +  \tfrac{c_0}{4}\; \BIR_2(t).
\end{align}
\end{theorem}

\begin{proof}[Proof Sketch]
We follow the steps in the proof of Theorem~\ref{thm:random-clean} to derive \begin{align*}
\PMR_1(t) - \PMR_2(t)
    &\geq \BIR_2(t)/2 -q,
    \quad \text{where $q = \exp(-\eps_0 t/12)$.}
\end{align*}
This is at least $\BIR_2(t)/4$ by \eqref{eq:random-assn}. Then \eqref{eq:thm:SoftMax-weak} follows by the smoothness condition \eqref{eq:SoftMax-smooth}.
\end{proof}

We recover a version of Corollary~\ref{cor:random}, if each principal's utility is the number of users (rather than the more general model in \eqref{eq:general-utility}). We also need a mild technical assumption that cumulative Bayesian regret (\BReg) tends to infinity. \BReg is a standard notion from the literature (along with \BIR):
\begin{align}\label{eq:SoftMax-BReg}
\BReg(n) := n\cdot \E_{\mu\sim\priorMu}
    \left[ \max_{a\in A} \mu_a\right] - \sum_{n=1}^n \rew(n')
    = \sum_{n'=1}^n \BIR(n').
\end{align}

\begin{corollary}\label{cor:SoftMax}
Assume that the response function is \SoftMaxRandom, and each principal's  utility is the number of users.
%
%Suppose principals can only choose algorithms from $\mA\cup \{\alg\}$, where $\mA\cup \{\alg\}$ is a finite set of monotone MAB algorithms such that each algorithm in $\mA$ satisfies \eqref{eq:random-assn} and $\BReg(n)\to \infty$, and is ``dominated" by \alg in the sense of \eqref{eq:random-better-messy}.
%
Consider the restricted competition game with special algorithm \alg, and assume that all other allowed algorithms satisfy $\BReg(n)\to \infty$. Then, for any sufficiently large time horizon $T$, this game has a unique Nash equilibrium: both principals choose \alg.
\end{corollary}

Further, we prove a much more challenging result in which the
condition \eqref{eq:random-better-weaker} is replaced with a much
weaker ``BIR-dominance'' condition. For clarity, we will again assume
that both algorithms are well-defined for an infinite time
horizon. The \emph{weak BIR dominance} condition says there exist
constants $\beta_0, \alpha_0\in (0, 1/2)$ and $n_0$ such that
 \begin{align}\label{eq:SoftMax-better}
   (\forall n\geq n_0) \quad
   \frac{\BIR_1((1-\beta_0)\, n)}{\BIR_2(n)} <1-\alpha_0.
 \end{align}
% for some $n_0(T)\in \polylog(T)$ and constants
% $\beta_0,\alpha_0\in (0, 1/2)$,
% \begin{align}\label{eq:SoftMax-better}
% (\forall n\geq n_0(T)) \quad
% \frac{\BIR_1((1-\beta_0)\, n\mid T)}{\BIR_2(n\mid T)} <1-\alpha_0.
% \end{align}
 If this holds, we say that \alg[1] \emph{weakly BIR-dominates}
 \alg[2]. Note that the condition \eqref{eq:random-better-messy}
 involves sufficiently small multiplicative factors (resp., $\eps_0/2$
 and $\tfrac12$), the new condition replaces them with factors that
 can be arbitrarily close to $1$.

 We make a mild assumption on \alg[1] that its $\BIR_1(n)$ tends to
 0. Formally, for any $\eps > 0$, there exists some $n(\eps)$ such
 that
 \begin{align}\label{eq:so-mild}
   (\forall n\geq n(\eps)) \qquad \BIR_1(n) \leq \eps.
 \end{align}
 We also require a slightly stronger version of the technical
 assumption~\eqref{eq:random-assn}:%  for any $\eps > 0$, there exists
 % $n(\eps)$ such that for
for some $n_0$,
\begin{align}\label{eq:SoftMax-assn-strong}
 % (\forall n\geq n(\eps)) \qquad
 %  \BIR_2(n) > e^{-\eps n}. %used to be 4exp( -\eps n/6)
(\forall n\geq n_0) \qquad 
\BIR_2(n) \geq \frac{4}{\alpha_0} \exp \left( \frac{-\min\{\eps_0, 1/8\} n}{12}\right)
\end{align}




\begin{theorem}\label{thm:SoftMax-strong}
  Assume the \SoftMaxRandom response function. Suppose \alg[1]
  weakly-BIR-dominates \alg[2], \alg[1] satisfies \eqref{eq:so-mild},
  and \alg[2] satisfies \eqref{eq:SoftMax-assn-strong}. Then there
  exists some $t_0$ such that each agent $t\geq t_0$ chooses principal
  $1$ with probability
\begin{align}\label{eq:thm:SoftMax-strong}
     \Pr[i_t = 1]\geq \tfrac12 +  \tfrac{c_0\alpha_0}{4}\; \BIR_2(t).
\end{align}
\end{theorem}




The main idea behind our proof is that even though \alg[1] may have a slower rate of learning in the beginning, it will gradually catch up
and surpass \alg[2]. We will describe this process in two phases. In
the first phase, \alg[1] receives a random agent with probability at
least $\respF(-1) = \eps_0$ in each round. Since $\BIR_1$ tends to 0,
the difference in \BIR{s} between the two algorithms is also
diminishing. Due to the \SoftMaxRandom response function, \alg[1]
attracts each agent with probability at least $1/2 - O(\beta_0)$ after
a sufficient number of rounds. Then the game enters the second phase:
both algorithms receive agents at a rate close to $\tfrac12$, and the
fractions of agents received by both algorithms --- $n_1(t)/t$ and
$n_2(t)/t$ --- also converge to $\tfrac12$. At the end of the second
phase and in each global round afterwards, the counts $n_1(t)$ and
$n_2(t)$ satisfy the weak BIR-dominance condition, in the sense that
they both are larger than $n_0$ and $n_1(t)\geq (1-\beta_0)\; n_2(t)$.
At this point, \alg[1] actually has smaller $\BIR$, which reflected in the {\PMR}s eventually. Accordingly, from then on \alg[1]
attracts agents at a rate slightly larger than $\tfrac12$. We prove
that the ``bump'' over $\tfrac12$ is at least on the order of
$\BIR_2(t)$. The detailed proof is deferred to the appendix.

Similar to the condition \eqref{eq:random-better-weaker}, we can also
generalize the weak BIR-dominance condition \eqref{eq:SoftMax-better}
to handle the dependence on $T$: there exist some $T_0$, a function
$n_0(T)\in \polylog(T)$, and constants $\beta_0,\alpha_0\in (0, 1/2)$, such that 
\begin{align}\label{eq:SoftMax-better-weaker}
(\forall T\geq T_0,  n\geq n_0(T)) \quad
\frac{\BIR_1((1-\beta_0)\, n\mid T)}{\BIR_2(n\mid T)} <1-\alpha_0.
\end{align}

We also provide a version of Theorem~\ref{thm:SoftMax-weak} under this
more general weak BIR-dominance condition; its proof is very similar
and is omitted. The following is just a direct consequence of
Theorem~\ref{thm:SoftMax-weak} with this general condition



\begin{corollary}\label{cor:SoftMax-strong}
Assume that the response function is \SoftMaxRandom, and each principal's  utility is the number of users. Consider the restricted competition game in which the special algorithm \alg weakly-BIR-dominates the other allowed algorithms, and the latter satisfy $\BReg(n)\to \infty$. Then, for any sufficiently large time horizon $T$, there is a unique Nash equilibrium: both principals choose \alg.
\end{corollary}


%If both $\BIR_1()$ and $\BIR_2()$ are of the form $\tilde{\Theta}(n^{-\gamma})$, $\gamma>0$, then the old condition requires $\BIR_1(\cdot)$ to be better by constant multiplicative factor $C$, with $C$ sufficiently large, whereas the new condition allows any $C>1$.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> itcs18paper/sec-welfare.tex <==
\asedit{We frame our contributions in terms of the relationship between \competitiveness and \rationality on one side, and adoption of better algorithms on the other. Recall that both \competitiveness (of the game between the two principals) and \rationality (of the agents) are controlled by the response function $\respF$.}

\OMIT{ %%%%%%
We frame our contributions in terms of the relationship between \competition and \innovation, \ie between the extent to which the game between the two principals is competitive, and the degree of innovation --- adoption of better that these models incentivize. \Competition is controlled via the response function $\respF$, and \innovation refers to the quality of the technology (MAB algorithms) adopted by the principals. The \competition vs. \innovation relationship is well-studied in the economics literature, and is commonly known to often follow an inverted-U shape, as in \reffig{fig:inverted-U} (see Section~\ref{sec:related-work} for citations). \Competition in our models is closely correlated with \rationality: the extent to which agents make rational decisions, and indeed \rationality is what $\respF$ controls directly.
} %%%%%%%%

\xhdr{Main story.}
Our main story concerns the restricted competition game between the two principals where one allowed algorithm \alg is ``better" than the others. \asedit{We track whether and when \alg is chosen in an equilibrium.} We vary \competitiveness/\rationality by changing the response function from \HardMax (full rationality, very competitive environment) to \HardMaxRandom to  \SoftMaxRandom (less rationality and competition). Our conclusions are as follows:
\begin{OneLiners}
\item Under \HardMax, no innovation: \DynGreedy is chosen over \alg.
\item Under \HardMaxRandom, some innovation:  \alg is chosen as long as it BIR-dominates.
\item Under \SoftMaxRandom, more innovation: \alg is chosen as long as it weakly-BIR-dominates.%
\footnote{This is a weaker condition, the better algorithm is chosen in a broader range of scenarios.}
\end{OneLiners}
These conclusions follow, respectively, from Corollaries~\ref{cor:DG-dominance}, \ref{cor:random} and \ref{cor:SoftMax}. Further, \asedit{we consider the uniform choice between the principals. It corresponds to the least amount of rationality and competition, and (when principals' utility is the number of agents) uniform choice provides no incentives to innovate.}%
\footnote{On the other hand, if principals' utility is somewhat aligned with agents' welfare, as in \eqref{eq:general-utility}, then a monopolist principal is incentivized to choose the best possible MAB algorithm (namely, to minimize cumulative Bayesian regret $\BReg(T)$). Accordingly, monopoly would result in better social welfare than competition, as the latter is likely to split the market and cause each principal to learn more slowly. This is a very generic and well-known effect regarding economies of scale.}
Thus, we have an inverted-U relationship, see \reffig{fig:inverted-U2}.


\begin{figure}
\begin{center}
\begin{tikzpicture}[scale=1]
      \draw[->] (-.5,0) -- (9.5,0) node[above] 
        {\qquad\qquad Competitiveness/Rationality};
      \draw[->] (0,-.5) -- (0,3) node[above] {Better algorithm in equilibrium};
      \draw[scale=0.8,domain=0.5:9.5,smooth,variable=\x,blue, line width=0.3mm] plot ({\x},{3.5 - 0.15*(\x - 5)^2});
     \node[below] at (1, 0) {\footnotesize \Uniform};
     \node[below] at (3.9, 0) {\footnotesize \SoftMaxRandom};
     \node[below] at (6, 0) {\footnotesize \HardMaxRandom};
     \node[below] at (8, 0) {\footnotesize \HardMax};
      % \draw[scale=0.5,domain=-3:3,smooth,variable=\y,red]  plot ({\y*\y},{\y});
 \end{tikzpicture}

\caption{The stylized inverted-U relationship in the ``main story".}
\label{fig:inverted-U2}
\end{center}
\end{figure}


\xhdr{Secondary story.}
Let us zoom in on the symmetric  \HardMaxRandom model. \asedit{Competitiveness and rationality within this model are controlled by the baseline probability $\eps_0 = \respF(- 1)$, which goes smoothly between the two extremes of \HardMax ($\eps_0=0$) and the uniform choice ($\eps_0=\tfrac12$). Smaller $\eps_0$ corresponds to increased rationality and increased competitiveness.} For clarity, we assume that principal's utility is the number of agents.

We consider the marginal utility of switching to a better algorithm. Suppose initially both principals use some algorithm \alg, and principal 1 ponders switching to another algorithm \alg' which BIR-dominates \alg. \asedit{We are interested in the marginal utility of this switch. Then:}

\begin{itemize}
\item $\eps_0 = 0$ (\HardMax):~~~~ the marginal utility can be negative if \alg is \DynGreedy.

\item $\eps_0$ near $0$:~~~~ only a small marginal utility can be guaranteed, as it may take a long time for $\alg'$ to ``catch up" with \alg, and hence less time to reap the benefits.

\item ``medium-range" $\eps_0$:~~~~ large marginal utility, as $\alg'$ learns fast and gets most agents.

\item $\eps_0$ near $\tfrac12$:~~~~ small marginal utility, as principal 1 gets most agents for free no matter what.
\end{itemize}
The familiar inverted-U shape is depicted in Figure~\ref{fig:inverted-U3}.



\begin{figure}
\begin{center}
\begin{tikzpicture}[scale=1]
      \draw[->] (-.5,0) -- (9.5,0) node[above]  {$\eps_0$};
      \draw[->] (0,-.5) -- (0,3) node[above] {marginal utility};
      \draw[scale=0.8,domain=0.5:9.5,smooth,variable=\x,blue, line width=0.3mm] plot ({\x},{3.5 - 0.15*(\x - 5)^2});
     \node[below] at (.6, 0) {\footnotesize \Uniform};
     \node[above] at (.5, 0) {\footnotesize 0};
     % \node[below] at (3.9, 0) {\footnotesize \SoftMaxRandom};
     % \node[below] at (6, 0) {\footnotesize \HardMaxRandom};
     \node[below] at (7.5,0) {\footnotesize \HardMax};
     \node[above] at (7.5, 0) {\footnotesize 1/2};
      % \draw[scale=0.5,domain=-3:3,smooth,variable=\y,red]  plot ({\y*\y},{\y});
 \end{tikzpicture}

\caption{The stylized inverted-U relationship from the ``secondary story"}
\label{fig:inverted-U3}
\end{center}
\end{figure}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

